flexBART: Flexible Bayesian regression trees with categorical predictors

Most implementations of Bayesian additive regression trees (BART) one-hot encode categorical predictors, replacing each one with several binary indicators, one for every level or category. Regression trees built with these indicators partition the discrete set of categorical levels by repeatedly removing one level at a time. Unfortunately, the vast majority of partitions cannot be built with this strategy, severely limiting BART's ability to partially pool data across groups of levels. Motivated by analyses of baseball data and neighborhood-level crime dynamics, we overcame this limitation by re-implementing BART with regression trees that can assign multiple levels to both branches of a decision tree node. To model spatial data aggregated into small regions, we further proposed a new decision rule prior that creates spatially contiguous regions by deleting a random edge from a random spanning tree of a suitably defined network. Our re-implementation, which is available in the flexBART package, often yields improved out-of-sample predictive performance and scales better to larger datasets than existing implementations of BART.

==> additional_experiments.tex <==

\subsection{Called strike probabilities}
\label{sec:pitchFraming_extra}

In Section 4.1 of the main text, we reported the in- and out-of-sample misclassification rates averaged over all 70 training and testing folds of our baseball data.
Figure~\ref{fig:pitch_framing_results} shows boxplots comparing three different error metrics --- misclassification rate, mean square error, and log-loss --- computed on each fold.
Each error metric was computed using the posterior mean estimate of the called strike probability.
We included the errors for the model that estimates called strike probability using pitch location only but omitted the out-of-sample results for \texttt{BART-alt} as those tended to be substantially larger than those of other methods.
We found that across all error metrics, \texttt{flexBART} achieved smaller error than \texttt{BART-default} and the location-only model on every training and testing fold.

%We have omitted the out-of-sample results for the method \texttt{BART-alt} as they tended to be substantially larger than the errors for all other methods.

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/pitchFraming_misclass_train}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/pitchFraming_mse_train}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/pitchFraming_logloss_train}
\end{subfigure}

\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/pitchFraming_misclass_test}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/pitchFraming_mse_test}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/pitchFraming_logloss_test}
\end{subfigure}
\caption{The misclassification rate, mean square error, and log-loss of \texttt{BART-default}, \texttt{BART-alt}, \texttt{flexBART}, and the location-only BART model on every training (top row) and testing (bottom row) fold. Out-of-sample errors for \texttt{BART-alt} were consistently much larger than those of other methods and were omitted from the figure.}
\label{fig:pitch_framing_results}
\end{figure}


\subsection{Philadelphia crime data}

In Section 4.2 of the main text, we reported the results of a leave-one-out analysis of the Philadelphia crime data.
In that experiment, we repeatedly trained a BART model using all data from $n -1 = 383$ census tracts and attempted to predict all the observations in the held-out tract.
We found that \texttt{networkBART}, a version of the BART prior that recursively partitioned the network of census tracts into spatially contiguous clusters, performed the best.
Essentially \texttt{networkBART} made predictions at the held-out tract by averaging predictions made in neighboring tracts.
Given the spatial smoothness evident in Figure 1a of the main text, our leave-one-out experiment arguably favors \texttt{networkBART} over \textbf{BART}-based implementations, which cannot exploit the spatial structure.
%Put another way, in view of the \textbf{BART} implementations averaging across all tracts, it is not especially surprising that \texttt{networkBART} performed better.

For an arguably fairer comparison, we performed a second cross-validation experiment in which we repeatedly trained BART models using 90\% of all observed data and evaluated the predictions on the remaining 10\%.
We held out data uniformly at random, ensuring that every census tract appeared in every training dataset, and allowing us to probe how partially pooling data across a network helps predict at vertices already seen during training. 

Figure~\ref{fig:philly_cv_rmse} compares the in- and out-of-sample RMSEs of each method across 100 different training-testing folds.
In this experiment, \texttt{BART-default} and \texttt{BART-alt} performed virtually identically, which is not entirely unexpected.
To elaborate, because every tract appeared in every training dataset, \texttt{BART-default} and \texttt{BART-alt} constructed identical internal design matrices for the training and testing data, which were subsequently passed to the same sampler. 

\begin{figure}[ht]
\centering
\begin{subfigure}[b]{0.4\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/philly_cv_rmse_train}
\caption{}
\label{fig:philly_cv_rmse_train}
\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/philly_cv_rmse_test}
\caption{}
\label{fig:philly_cv_rmse_test}
\end{subfigure}
%\includegrapics[width = \textwidth]{figures/philly_cv_rmse}
\caption{In-sample (a) and out-of-sample (b) RMSE across 100 training-testing splits of the crime data.}
\label{fig:philly_cv_rmse}
\end{figure}

Similar to what we observed in the leave-one-out experiment from Section 4.2 of the main text, our second experiment reveals that pooling data across multiple census tracts can improve predictions.
However, unlike that experiment, Figure~\ref{fig:philly_cv_rmse_test} reveals that \texttt{networkBART} and \texttt{flexBART} achieved extremely similar out-of-sample RMSEs.
That is, while leveraging the adjacency structure helped in our leave-one-out experiment, in our second experiment, \textit{how} we partially pooled data did not make a material difference.
While these finds appear to contradict one another, they actually align with our basic intuition about Bayesian shrinkage.
Namely, when partially pooling across many groups, the effects of shrinkage are more apparent for groups with very little data.
Recall that no data was observed in the held-out tract during training in our leave-one-out experiment.
As a result, the effects of our network-informed shrinkage are quite evident there.
By contrast, in our second experiment, because we observed quite a lot of data from each tract during training, we would not expect to see much evidence of shrinkage. 

==> bart_review.tex <==
\citet{Chipman2010} introduced BART in the context of the general nonparametric regression problem: given $n$ observations of a pair of a $p$-dimensional covariate vector $\bx$ and a scalar output $y$ that are modeled as $y \sim \normaldist{f(\bx)}{\sigma^{2}},$ we want to learn the regression function $f.$
We briefly review the basic BART model in the setting where all $p$ covariates are continuous and lie, without loss of any generality, in the interval $[0,1]$.   
BART works by approximating $f$ as a sum of $M$ binary regression trees, specifying a prior over the collection of trees, and then computing a posterior distribution over tree ensembles, which in turn induces an approximate posterior distribution over the function $f.$

\subsection{A sum-of-trees model}
\label{sec:regression_trees}
A \textit{regression tree} is a triplet $(T, \calD, \bmu)$ consisting of (i) a finite rooted binary tree $T$ containing $L(T)$ terminal or \textit{leaf nodes} and a collection of non-terminal nodes; (ii) a collection of decision rules $\calD,$ one for each non-terminal node in $T;$ and (iii) a collection $\bmu$ of $L(T)$ scalars or \textit{jumps}, one for each leaf node in $T.$
When $T$ contains a non-root node, every non-terminal node $\nx$ is connected to two \textit{children}, which we refer to as the left and right child of $\nx.$
%We can additionally label each node in $T$ with a positive integer in a recursive fashion: after labeling the root with 1, we can respectively label the left and right child of a node labelled $k$ with $2k$ and $2k+1.$
%Note that these labels induce a natural ordering on the non-terminal nodes and separately induce an ordering on the leafs.

The basic BART model parametrizes the decision rule associated the non-terminal node $\nx$ with a pair $(v(\nx),c(\nx)),$ where $v(\nx) \in \{1,2, \ldots, p\}$ is the \textit{splitting variable index} and $c(\nx) \in [0,1]$ is the \textit{cutpoint}. 
For every $\bx = (x_{1}, \ldots, x_{p}) \in [0,1]^{p},$ we can trace a path from the root of $T$ to exactly one leaf node as follows.
Starting from the root, once the path reaches the non-terminal node $\nx,$ it proceeds to the left child of $\nx$ if the $v(\nx)$-th coordinate of $\bx$ is less than $c(\nx)$ (i.e.~if $x_{v(\nx)} < c(\nx)$) and to the right child of $\nx$ otherwise (i.e.~if $x_{v(\nx)} \geq c(\nx)$).
The decision-following path for each $\bx$ terminates at a single leaf node.
By associating each point $\bx \in [0,1]^{D}$ with exactly one of the $L(T)$ leaf nodes, the \textit{decision tree} $(T,\calD)$ partitions $[0,1]^{p}$ into $L(T)$ disjoint sets, one for each leaf node.
In fact, these sets are axis-parallel rectangular boxes.
By associating each leaf $\ell$ with a scalar jump $\mu_{\ell} \in \R,$ the regression tree $(T, \calD, \bmu)$ represents a piecewise constant step function (see Figure~\ref{fig:sum_of_trees} for several examples).

\begin{figure}[ht]
\centering
\includegraphics[width = \textwidth]{figures/sum_of_trees}
\caption{The sum of regression trees is also a regression tree whose jumps are sums of jumps from each tree in the ensemble. Relatively smooth functions can be well-approximated using ensembles of rather simple, discontinuous step functions}
\label{fig:sum_of_trees}
\end{figure}

BART represents unknowns functions using a sum of $M$ \textit{a priori} independent regression trees.
Because the total number of parameters, which include all of the tree structures, decision rules, and jumps, increases rapidly with $M,$ taking $M$ to be large endows BART with tremendous representational flexibility.
Indeed, \citet{Chipman2010} recommended using $M = 200$ regression trees as a default.
As Figure~\ref{fig:sum_of_trees} suggests, rather complicated functions, which might be represented with a single deep tree with many leaf nodes, can usually be written as a sum of simple regression trees containing only a few leaf nodes.
Accordingly \citet{Chipman2010} specified a regression tree prior that aggressively regularized towards shallow trees containing a small number of leaves.

\subsection{The default BART regression tree prior}
\label{sec:cgm10_prior}

\citet{Chipman2010} specified their regression tree prior implicitly using a stochastic process for simulating prior draws.
We can describe the prior tree-drawing process using three steps. 
In the first step, the process samples the tree $T$ using a branching process first described in \citet{Chipman1998}.
Then, conditionally on $T,$ the process sequentially draws random decision rules at each non-terminal node.
Finally, conditionally on $T,$ the process draws the $L(T)$ jumps in $\bmu$ independently from a $\normaldist{0}{\tau^{2}/M}$ distribution.

\textbf{Drawing $T$}. \citet{Chipman1998}'s branching process grows $T$ in a recursive fashion starting from a single root node, which is considered to be a terminal node of depth zero.
Each time a new terminal node is created at depth $d$, the branching process grows the tree from that node by adding two children nodes with probability $0.95(1 + d)^{-2}.$
Because the probability that the process continues growing decays quadratically with tree depth, the branching process terminates with finitely many leaves.

\textbf{Drawing $\calD \vert T$}. The decision rule at non-terminal node $\nx$ is drawn in two steps. 
First, the splitting variable index $v(\nx)$ is drawn uniformly from the set $\{1,2,\ldots, p\}.$
Then, conditionally on $v(\nx),$ $c(\nx)$ is drawn uniformly from a set $\calA(v(\nx),\nx)$ that contains all values of the $v(\nx)$-th covariate available at the node $\nx.$
The decision rules associated with the ancestors of $\nx$ in the tree fully determine the set $\calA(v(\nx),\nx).$
Conceptually, we could compute $\calA(v(\nx), \nx)$ by scanning over all $\bx \in [0,1]^{p}$ and adding $x_{v(\nx)}$ to the set if $\bx$'s decision-following path reaches $\nx.$
In practice, we can quickly compute $\calA(v(\nx), \nx)$ by recursing up the tree from $\nx$ to the root and taking appropriate set intersections.

\begin{remark}
Before proceeding, we pause to note that the three-step tree-drawing process described above differs slightly from the process described in \citet[\S 2.2]{Chipman2010}.
In their process, decision rules are drawn as part of the tree-generating branching process.
Practically, simultaneously growing $T$ and $\calD$ is equivalent to first drawing $T$ and then conditionally drawing $\calD$ as we describe.
%The deliberate separation of the structure of the tree $T$ (i.e. the overall arrangement of the leafs and edges) from the decision rules $\calD$, both in our notation and description of the prior, will make it easier to describe the modifications we make to BART in Section~\ref{sec:flex_bart}.
\end{remark}

When all $p$ covariates are continuous, the set $\calA(v(\nx), \nx)$ will be an interval.
By drawing $c(\nx) \in \calA(v(\nx), \nx),$ we ensure that (i) each non-trivial node is visited by the decision-following path of at least one $\bx \in [0,1]^{p}$ and (ii) the decision tree $(T,\calD)$ partitions $[0,1]^{p}$ into exactly $L(T)$ axis-parallel rectangular boxes.
In this way, the default regression tree prior used by BART induces a prior over the space of partitions of $[0,1]^{p}$ into such boxes.
It turns out, moreover, the induced prior on partitions places positive density on every such partition of $[0,1]^{p}.$
Coupled with the absolutely continuous $\normaldist{0}{\tau^{2}/M}$ prior on the jumps, the regression tree prior places positive density on essentially every piecewise constant step function.

\begin{remark}
Whereas we allow cutpoints $c(\nx)$ to be drawn uniformly from an interval, \citet{Chipman2010} restrict cutpoints to the set of observed covariate values. 
Their implementation in the \textbf{BART} package \citep{BART_package} further truncates the prior to those trees in which every leaf node is reached by the decision-following path of at least five observations\footnote{The restriction is enforced on line 47 of the internal \texttt{bd()} function \href{https://github.com/cran/BART/blob/master/src/bd.cpp\#L47}{here}.}.
Such restrictions sacrifice Bayesian coherence and place zero prior probability on regression trees whose cutpoints lie outside the set of observed covariate values.
The prior described above, in contrast, makes no such restrictions, thereby retaining Bayesian coherence and the desirable full support property.
\end{remark}

\subsection{Posterior computation}
\label{sec:backfitting}

\citet{Chipman2010} proposed a Gibbs sampling strategy to simulate posterior samples of the regression tree ensemble.
In each iteration, each regression tree is updated conditionally fixing the remaining $M-1$ trees.
Two steps are used to update individual regression trees.
First, a new decision tree $(T,\calD)$ is drawn from its conditional posterior distribution given the remaining $M-1$ regression trees and the data.
Then, a new collection of jumps $\bmu$ is drawn from its conditional posterior distribution given the just-drawn decision tree $(T, \calD),$ the other $M-1$ regression trees, and the data.

The new decision tree $(T,\calD)$ is drawn with a Metropolis-Hasting (MH) step.
While there are several proposal distributions encouraging both small and large modifications to both $T$ and $\calD$ \citep[see, e.g.,][]{Pratola2016, Mohammadi2020}, we here focus on a simple proposal distribution that either randomly prunes or grows the decision tree.
Pruning $(T,\calD)$ involves (i) deleting two leaf nodes that share a common parent, which is selected uniformly at random, and their incident edges in $T$; (ii) deleting the decision rule associated with the parent of the deleted leaf nodes; and (iii) leaving the rest of the tree and decision rules unchanged.
Growing $(T,\calD)$ in contrast, involves (i) adding two nodes to the tree and connecting them to an existing leaf node selected uniformly at random; (ii) drawing a decision rule for the selected node; and (iii) leaving the rest of the tree and decision rules unchanged.
For simplicity, when growing a tree, we draw the decision rule for the newly-created non-terminal node from the prior introduced in Section~\ref{sec:cgm10_prior}; that is, we (i) draw the splitting variable index uniformly and (ii) uniformly draw a cutpoint from the interval of covariate values available at the node.

==> flex_bart.tex <==
When all $p$ covariates are continuous and lie in the unit interval, the default BART prior described in Section~\ref{sec:cgm10_prior} places (i) positive density on every partition of $[0,1]^{p}$ into disjoint axis-parallel rectangular boxes and (ii) positive density on every piecewise constant function defined over such partitions. 
Together, these full support properties endow BART with tremendous flexibility: basically, BART is not prevented \textit{a priori} from using any given step function to approximate $f(\bx).$

However, as we will demonstrate in Section~\ref{sec:partition_problem}, when categorical covariates are converted into binary indicators, the default BART prior places zero prior probability on a staggeringly overwhelming majority of partitions of the covariate space, which is the product of continuous and unordered discrete spaces.
Consequently, BART is prevented from using the great majority of step functions defined over the covariate space to help approximate $f,$ severely diminishing its representational capacity. 
In Section~\ref{sec:new_rules}, we propose a simple modification --- namely a more general type of decision rule --- that substantially expands the representational capacity of BART's regression tree ensemble.

\subsection{A binary indicator-induced hole in the BART prior}
\label{sec:partition_problem}

Consider, for the moment, a setting with no continuous covariates and only one categorical covariate $X$ that takes values in $\{\lambda_{1}, \ldots, \lambda_{K}\}.$
By default, BART operationalizes the predictor by introducing $K$ binary indicators, $X_{1}, \ldots, X_{K},$ where $X_{k} = \ind{X = \lambda_{k}}$ for each $k = 1, \ldots, K.$
Suppose that $(T, \calD, \bmu)$ is a regression tree with at least two leaf nodes drawn using the three-step process described in Section~\ref{sec:cgm10_prior}.
Since the decision tree $(T,\calD)$ partitions the entire space $[0,1]^{D}$, it automatically partitions the set of standard basis vectors $\{\bm{e}_{1}, \ldots, \bm{e}_{K}\}$ where the $k$-th entry of $\bm{e}_{k}$ is equal to one and all other entries are equal to zero.
Since we can identify $\bm{e}_{k}$ with the level $\lambda_{k}$ of $X,$ we conclude that the decision tree $(T, \calD)$ partitions the levels of $X.$
In fact, $(T, \calD)$ partitions the levels of $X$ into several singleton sets with one level each and at most one set with multiple levels.
Figure~\ref{fig:philly_remove_one} shows two such examples of the partitions of the Philadelphia census tracts induced by the default BART prior.
Both of these partitions feature one large set of tracts and some singleton sets.

To understand why the default prior can produce only such partitions, consider the decision-following paths for each of the $\mathbf{e}_{k}$'s.
Without loss of generality, suppose the splitting variable index at the root is 1.
Because the first coordinates of $\mathbf{e}_{2}, \ldots, \mathbf{e}_{K}$ are all zero, the paths for these $K-1$ points will proceed to the left child of the root while the path for $\mathbf{e}_{1}$ will proceed to the right child.
Consequently, when partitioning the points $\{\mathbf{e}_{1}, \ldots, \mathbf{e}_{K}\},$ the tree separates $\mathbf{e}_{1}$ in a singleton set away from the other $K-1$ points.
At every subsequent non-terminal node, at most one path can proceed to the right child while all others proceed to the left child. 
In this way, by tracing the decision-following paths of the $\mathbf{e}_{k}$'s, we see that the decision tree $(T,\calD)$ recursively partitions the set $\{\lambda_{1}, \ldots, \lambda_{K}\}$ by removing at most one element at a time.
Ultimately, then, the default BART prior places positive probability on only those partitions that can formed by recursively removing at most one element at a time.

%Such a recursive ``remove (at most) one at a time'' process cannot partition the set $\{\lambda_{1}, \ldots, \lambda_{K}\}$ into multiple sets containing more than one element each.
%Rather, such process can only produce the $2^{K} - K$ partitions containing several singleton sets and at most one set with multiple elements. 

\begin{figure}[ht]

\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/philly_remove_one_annotate}
\caption{}
\label{fig:philly_remove_one}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/philly_uniform_unordered_annotate}
\caption{}
\label{fig:philly_uniform_unordered}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/philly_spanning_tree_annotate}
\caption{}
\label{fig:philly_spanning_tree}
\end{subfigure}
\caption{Examples of partitions of the Philadelphia census tracts induced by regression trees drawn using (a) the default BART prior's ``remove one at a time'' strategy, (b) our new prior with the uniform unordered process, and (c) our new prior with the uniform spanning tree process. In each example, we have colored the census tracts according to their corresponding leaf in the regression tree.}
\label{fig:philly_partitions}
\end{figure}


%Such a recursive ``remove (at most) one at a time'' process can only produce the $2^{K} - K$ partitions containing at most one set with multiple elements and possibly some singleton sets.
%This means that the default BART prior places positive probability on only $2^{K} - K$ partitions
It turns out that there are only $2^{K} - K$ such partitions.
When $X$ contains more than two levels (i.e.~$K > 2$), this number is much smaller than the total number of partitions of $K$ objects (i.e.~the $K$-th Bell number; \citet[pg.~33]{Stanley_enum}).
For instance, when $K = 5,$ the default BART prior places positive probability on only 27 of the 52 possible partitions and when $K = 10,$ the default BART prior supports less than 1\% of all possible partitions (1,014 versus 115,975).
So by converting the inherently discrete and unordered $X$ into several continuous ordered covariates, the default BART prior places zero probability on a potentially enormous number of partitions of the levels of $X.$

\subsection{A new class of decision rules}
\label{sec:new_rules}

The argument in Section~\ref{sec:partition_problem} extends naturally to more realistic settings featuring both continuous and categorical predictors.
Namely, if we convert each categorical predictor into binary indicators, the default BART prior place positive density on an extremely narrow range of step functions defined over the covariate space, which is a product of continuous and unordered discrete spaces.
Consequently, BART is severely limited in its ability to model functions that display similar variation over multiple levels of a categorical predictor.
Concretely, in the crime modeling problem, BART cannot include functions that are constant within each of the circled regions of Figure~\ref{fig:philly_means} in the ensemble.

To expand BART's flexibility when some covariates are categorical, we recommend against one-hot encoding categorical predictors.
Formally, suppose that we have $\pcont$ continuous predictors $X_{1}, \ldots, X_{\pcont}$ which, without loss of generality, lie in the interval $[0,1],$ and $\pcat$ categorical predictors $X_{\pcont +1}, \ldots, X_{p}$ where $p = \pcont + \pcat.$ 
Further suppose that the $j$-th categorical covariate $X_{\pcont + j}$ takes on $K_{j}$ values that are contained in the set $\calK_{j}.$
We wish to use BART to estimate a function $f: [0,1]^{\pcont} \times \calK_{1} \times \cdots \calK_{\pcat} \rightarrow \R$.
Observe that the covariate space is the product of continuous ordered spaces and discrete unordered spaces.
%Because some coordinates of the covariate vector $\bx \in [0,1]^{\pcont} \times \calK_{1} \times \cdots \times \calK_{\pcat}$ are unordered, we can no longer use the regression trees introduced in Section~\ref{sec:bart_review}.

Unfortunately, we can longer use the regression trees introduced in Section~\ref{sec:bart_review} for this purpose because the behavior of the decision-following paths described above is undefined when some coordinates of $\bx$ are unordered.
Fitting more flexible BART models with both continuous and unordered categorical covariates requires a more general class of decision rule.
Specifically, we instead work with decision rules $(v, \cutset),$ which are parametrized by a variable splitting index $v$ and a \textit{cutset} $\cutset.$
With such rules, we can trace a decision-following path from root to leaf for each $\bx \in [0,1]^{\pcont} \times \calK_{1} \times \cdots \times \calK_{\pcat}$ as follows.
Starting from the root, once the path reaches a non-terminal node $\nx,$ the path proceeds to the left child if $x_{v(\nx)} \in \cutset(\nx)$ and to the right child otherwise.

\textbf{A new decision rule prior}.
Fitting a BART model using regression trees with decision rules of the form $(v, \cutset)$ formally requires specifying (i) a prior over the new class of regression trees and (ii) a proposal distribution for updating decision trees $(T,\calD)$ with Metropolis-Hastings.
Insofar as we are only changing the decision rules, we will use exactly the same priors for the tree $T$ and jumps $\bmu \vert T$ described in Section~\ref{sec:cgm10_prior}.
We only introduce a new decision rule prior.
Further, just like in Section~\ref{sec:backfitting}, we only use grow and prune proposals in our Gibbs sampler and draw decision rules created during grow moves from our new prior.

Like before, we specify our new decision rule prior at non-terminal node $\nx$ implicitly by describing a process for simulating prior draws.  
At non-terminal node $\nx,$ we first draw the variable splitting index $v(\nx)$ uniformly as before.
Then, we compute $\calA(v(\nx), \nx)$, the set of available values for the $v(\nx)$-th predictor at node $\nx.$
To ensure that the resulting decision tree $(T,\calD)$ partitions the space $[0,1]^{\pcont} \times \calK_{1} \times \cdots \times \calK_{\pcat},$ we take $\cutset(\nx)$ to be a randomly drawn non-trivial subset of $\calA(v(\nx), \nx).$
That is, we draw $\cutset(\nx) \subset \calA(v(\nx),\nx)$ with the restriction that it is non-empty and not equal to $\calA(v(\nx), \nx).$

How we draw the cutset depends on whether the $v(\nx)$-th covariate is continuous or categorical.
Briefly, when the $v(\nx)$-th covariate is continuous, we draw the cutset using what we call the \textit{continuous uniform process}.
When the $v(\nx)$-th covariate is categorical, if we do not have an \textit{a priori} preference to co-cluster certain pairs of levels more often than others, we draw the cutset using what we call the \textit{uniform unordered process}.
On the other hand, if we specify a network encoding our co-clustering preferences, we draw the cutset using the \textit{uniform spanning tree process}.
%On the other hand, if we have encoded prior preferences about which levels of the $v(\nx)$-th covariate should be frequently co-clustered with a network, we draw the cutset using the \textit{uniform spanning tree process}.
We detail these processes in Section~\ref{sec:cutset_prior}.

\subsection{Conditional priors over cutsets $\cutset$}
\label{sec:cutset_prior}

\textbf{The continuous uniform process}.
When the $v(\nx)$-th covariate is continuous, $\calA(v(\nx),\nx)$ is an interval and we draw the cutset $\cutset(\nx)$ by first selecting $c \in \calA(v(\nx),\nx)$ uniformly and then setting $\cutset = \calA(v(\nx),\nx) \cap [0,c).$
This process produces exactly the same sorts of decision rules as the process described in Section~\ref{sec:cgm10_prior}.

\textbf{The uniform unordered process}. 
When the $v(\nx)$-th covariate is categorical, the set of available values $\calA(v(\nx),\nx)$ is discrete and we now must draw a non-trivial random subset $\cutset(\nx) \subset \calA(v(\nx), \nx).$
Arguably the simplest option is to sample $\cutset(\nx)$ uniformly from the set of all non-trivial subsets of $\calA(v(\nx), \nx),$ using what we call the discrete uniform process.
Practically, the process works by initializing $\cutset(\nx) = \emptyset$ and then sequentially adding elements of $\calA(v(\nx), \nx)$ to $\cutset(\nx)$ with probability 1/2.
If, at the end of this sweep, $\cutset(\nx)$ remains empty or is exactly $\calA(v(\nx), \nx),$ we reset $\cutset(\nx) = \emptyset$ and repeat the sweep until $\cutset(\nx)$ is non-trivial.

Because they induce partitions over the entire covariate space $[0,1]^{\pcont} \times \calK_{1} \times \cdots \times \calK_{\pcat},$ regression trees drawn from our new prior partition each of the discrete sets $\calK_{j}.$
In fact, our discrete uniform process ensures that the induced prior over partitions of $\calK_{j}$ places positive probability on all possible partitions, in sharp contrast to the ``remove at most one at a time'' process described in Section~\ref{sec:cgm10_prior}.
Figure~\ref{fig:philly_uniform_unordered} shows two examples of the partitions of the census tracts in Philadelphia induced by regression trees drawn using our new prior equipped with the uniform unordered process.
Unlike the partitions in Figure~\ref{fig:philly_remove_one}, partitions drawn from our new prior can contain multiple multi-element sets. 
By symmetry, each level of the categorical predictor is equally likely to be co-clustered with every other level.

\begin{remark}
Our uniform unordered process is biased towards drawing cutsets containing about half of the available levels.
Rather than fixing the probability of inclusion into $\cutset$ to be 0.5, a more general process would first sample the inclusion probability and then assign elements of $\calA$ to $\cutset$ with that probability.
Such generalization also places positive probability on all partitions of the sets of categorical levels.
\citet{Chipman1998} proposed exactly such a generalization in the prior underlying their single-tree Bayesian CART model.
Curiously, however, they later abandoned the prior in BART, opting instead for the more conventional binary encoding of categorical variables.
\end{remark}

\textbf{The uniform spanning tree process}. 
A closer examination of the partitions in Figure~\ref{fig:philly_uniform_unordered} reveals that the clusters of tracts are not spatially contiguous.
The resulting regression trees effectively pool data from geographically disparate census tracts.
In light of the spatial smoothness in Figure~\ref{fig:philly_means}, we might instead prefer spatially contiguous partitions like those in Figure~\ref{fig:philly_spanning_tree}, which only pool data from neighboring tracts.

When we have spatial data aggregated into areal units (e.g.~blocks, census tracts, states), we can represent the areas with a network $\calG$ whose vertices correspond to the areal units and whose edges encode spatial adjacencies.
Figure~\ref{fig:philly_graph} shows the adjacency network of the Philadelphia census tracts.
When modeling such areal data, we can represent location using the vertex label in $\calG$, which is a structured categorical variable. 
%To ensure regression trees partition the underlying geographic region into spatially contiguous partitions, we introduce the \textit{uniform spanning tree} process.

More generally, we might sometimes express \textit{a priori} preference that certain categorical levels be co-clustered more often than others, at odds with the symmetric nature of the uniform unordered process.
In these scenarios, we can represent those preferences using a network $\calG$ whose vertices are the levels of the categorical covariate.
We further draw edges in $\calG$ between the levels that we prefer to co-cluster.
In the crime modeling example, the network edges encode the preference that spatially adjacent tracts co-cluster more frequently together than non-adjacent tracts.
As evidenced by Figure~\ref{fig:philly_uniform_unordered}, recursive partitioning with the uniform unordered process tends to create partitions whose clusters do not induce connected subgraphs of $\calG.$
The following \textit{uniform spanning tree process} produces cutsets that more faithfully respect $\calG$'s connectivity.


Given a set of available levels $\calA$ at a non-terminal node, the uniform spanning tree process draws a random subset $\cutset \subset \calA$ such that both $\cutset$ and $\calA\setminus \cutset$ induce connected subgraphs of $\calG.$
The process works by partitioning $\calG[\calA],$ the subgraph of $\calG$ induced by $\calA,$ into two connected components.
Specifically the process first draws a spanning tree of $\calG[\calA]$ uniformly at random by performing a loop-erased random walk on the vertices of $\calG[\calA]$ \citep[i.e., we use Wilson's algorithm;][]{Wilson1996}.
Then it deletes a uniformly selected edge from the spanning tree, thereby partitioning the spanning tree into two connected components.
The process then assigns the vertices in one of these components to $\cutset.$
Figure~\ref{fig:mst_split} illustrates how our uniform spanning tree process works.

\begin{figure}[ht]
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_a}
\caption{}
\label{fig:mst_split_a}
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_b}
\caption{}
\label{fig:mst_split_b}
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_c}
\caption{}
\label{fig:mst_split_c}
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_d}
\caption{}
\label{fig:mst_split_d}
\end{subfigure}
\caption{Cartoon illustration of our uniform spanning tree process.(a) Induced subgraph of levels available at a particular non-terminal node in the decision tree. (b) Uniformly drawn random spanning tree. (c) Deleting a uniformly selected edge (the edge $(2,8)$ in this case) from the spanning tree disconnects the tree and partitions the vertices into two subsets. (d) The subgraphs induced by the two vertex sets produced in (c) remain connected.}
\label{fig:mst_split}
\end{figure}

Our regression tree prior with the uniform spanning tree process places positive probability on every partition of a network into finitely many connected components.
Our uniform spanning tree process follows an emerging trend in the spatial clustering literature that builds spatially contiguous partitions by deleting edges from spanning trees \citep[see, e.g.,][]{Teixeira2015, Teixeira2019, LiSang2019, Luo2021}.
In the context of Bayesian treed regression, \citet{Luo2021_BAST} and \citet{Luo2022} have recently introduced a decision rule prior that is very similar to our uniform spanning tree process.
Whereas we were motivated by categorical predictors displaying network structure, their procedure recursively partitions a continuous manifold.
Briefly, they first triangulate the manifold and form a graph whose vertices corresponding to the triangular regions and whose edges encode adjacency relationships between the regions. 
Then they recursively remove edges from spanning trees of the graph to partition the manifold into contiguous regions.

\begin{remark}
The uniform unordered and uniform spanning tree process adaptively construct new covariates on which a regression tree can split.
These new covariates have the form $\ind{x_{v} \in \cutset},$ which can be written as the sum of binary indicators corresponding to each element of $\cutset$ when $X_{v}$ is categorical.
In other words, these processes allow trees to split on new covariates formed by agglomerating multiple levels of a categorical covariate into a new covariate. 
Breiman similarly suggested randomly combining categorical levels in his random forests algorithm \citep[\S 5.1]{Breiman2001}.
\end{remark}

\subsection{Our new regression tree prior}

To summarize, our new regression trees are based on decision rules that send paths to the left if $x_{v} \in \cutset$ and to the right otherwise.
We draw the cutset $\cutset$ based on the type of the splitting variable at each non-terminal node.
When the splitting variable is continuous, we draw $\cutset$ from the uniform continuous process.
When the splitting variable is categorical, we use the uniform unordered process if we have no \textit{a priori} preferences about how the categorical levels ought to co-cluster.
We use the uniform spanning tree process if we have specified a network encoding co-clustering preferences amongst the levels.


==> flex_bart2.tex <==
Most BART implementations one-hot encode categorical predictors, replacing each with a collection of binary indicators, one for every level.
That is, rather than work with the original predictor space $\calX,$ which is a product of Euclidean and discrete spaces, they instead work with an extended predictor space $\tilde{X} = [0,1]^{\tilde{p}}$ where $\tilde{p} = \pcont + \lvert \calK_{1}\rvert + \cdots + \lvert \calK_{\pcat}\rvert.$
At first glance, one-hot encoding appears innocuous since no information about the predictor is lost.
Further, one-hot encoding is \textit{de rigueur} within statistics and machine learning, with many popular textbooks recommending the practice, especially for (generalized) linear modeling. 
In light of Remark~\ref{remark:continuous_full_support}, it would appear that by replacing categorical predictors with continuous ones, these BART implementations inherit desirable full support properties.

\subsection{A one-hot encoded hole in the BART prior}
\label{sec:partition_problem}

The situation is, regrettably, not quite so simple.
Although the prior places positive probability on every partition of the extended space $\tilde{\calX}$ into axis-parallel boxes, it places zero probability on a staggeringly overwhelming majority of partitions of the original space $\calX.$

To illustrate such lack-of-support, consider a setting with only one categorical predictor $X$ taking values in $\{c_{1}, \ldots, c_{K}\}.$
One-hot encoding $X$ introduces $K$ binary indicators, $X_{1}, \ldots, X_{K},$ where $X_{k} = \ind{X = c_{k}}.$ 
Suppose that $(T, \calD, \bmu)$ is a regression tree with at least two leaf nodes defined over the extended space $[0,1]^{K}.$
Since $(T,\calD)$ partitions the entire space $[0,1]^{K}$, it automatically partitions the set of standard basis vectors $\{\bm{e}_{1}, \ldots, \bm{e}_{K}\}$ where the $k$-th entry of $\bm{e}_{k}$ is equal to one and all other entries are zero.
By identifying $\bm{e}_{k}$ with the level $c_{k}$ of $X,$ we conclude that $(T, \calD)$ also partitions $X$'s levels.

In fact, $(T, \calD)$ partitions $X$'s levels into several singleton sets containing one level and at most one set containing multiple levels.
To understand why, consider the $\bm{e}_{k}$'s decision-following paths.
When they encounter the decision rule $\{X_{j} \in [0,c)\},$ only $\bm{e}_{j}$'s path can proceed to the right while all others proceed to the left.
Thus, the decision tree partitions $\{c_{1}, \ldots, c_{K}\}$ by repeatedly removing one element at a time.
Such a strategy can only produce $2^{K} - K$ distinct partitions of $\{c_{1}, \ldots, c_{K}\}.$
When $K > 2,$ this number is much smaller than the $K$-th Bell number, which counts the number of partitions of $K$ objects.
For instance, after one-hot encoding, the BART prior places positive probability on just 27 of the 52 possible partitions when $K = 5$ and on less than 1\% of partitions when $K = 10$ (1,014 out of 115,975).
The scale of this lack-of-support phenomenon is magnified in the presence of multiple predictors.
%By one-hot encoding categorical predictors, most BART implementations cannot partially pool data across small groups of levels.

Figure~\ref{fig:philly_remove_one} illustrates typical partitions of the Philadelphia census tracts supported by the BART prior after one-hot encoding.
The corresponding regression trees pool together data from most tracts into one big cluster while separately modeling a few singleton tracts.
Although such modeling may be desirable when all but a few census tracts display similar crime dynamics, it is wholly inadequate in light of Figure~\ref{fig:philly_crime_intro}.
Indeed, a cursory look at that figure suggests forming several small clusters containing multiple tracts with similar dynamics would be more effective.
Unfortunately, such clusters cannot be formed by the BART prior after one-hot encoding.

\begin{figure}[ht]

\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/remove_plots}
\caption{}
\label{fig:philly_remove_one}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/disc_unif_plots}
\caption{}
\label{fig:philly_uniform_unordered}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/ust_unif_plots}
\caption{}
\label{fig:philly_spanning_tree}
\end{subfigure}
\caption{Examples of partitions of the Philadelphia census tracts induced by regression trees drawn from (a) the BART prior after one-hot encoding; (b) without one-hot encoding and instead independently assigning levels to the left and right branches at random; and (c) using the network-based approach described in Section~\ref{sec:network_splits}. We colored the census tracts according to their corresponding leaf in the regression tree.}
\label{fig:philly_partitions}
\end{figure}

\subsection{A more flexible and extensible implementation}
\label{sec:implementation}

To overcome the limitations of one-hot encoding, we developed \textbf{flexBART}, a new implementation of BART that uses regression trees that can assign multiple levels to each branch to encourages richer partial pooling across categorical levels.
Figure~\ref{fig:new_tree} shows an example of such a tree defined over the space $\calX = [0,1]\times \left\{c_{1}, \ldots, c_{6}\right\}.$
In writing \textbf{flexBART}, we largely followed the example set by the authors of \textbf{BART}, writing \textbf{flexBART}'s core sampling functions in \textsf{C++} and interfacing those functions with \textsf{R} through \textbf{Rcpp} \citep{Rcpp}.
Although our overall design is similar to theirs, there are several key differences.
Briefly, we created a new, highly extensible class to represent decision rules and eliminated many redundant calculations performed by \textbf{BART}, which led to substantial run-time improvements.
\textbf{flexBART} is available at \url{https://github.com/skdeshpande91/flexBART}.

As described in \citet{Pratola2014_parallel}, \textbf{BART} represents regression trees as a collection of nodes, which are instances of a custom class containing only six data members: (i) pointers to separate class instances for the parent and children of the node; (ii) an integer for the decision variable index $j$; (iii) an integer recording the index of the cutpoint $c$\footnote{\textbf{BART} pre-computes a finite grid of cutpoints for each predictor instead of drawing them from $[0,1]$.}; and (iv) a double for the jump.
Armed with this lightweight class, \textbf{BART}'s authors wrote a recursive functions that traces the decision-following path of each $\bx \in \calX.$
Although the class and this function facilitate extremely fast and memory-efficient MCMC simulations, they are insufficient for representing regression trees like the one in Figure~\ref{fig:new_tree}.

We consequently re-wrote the regression tree node class and replaced the two integers parametrizing the decision rule with an instance of a new class representing decision rules.
The data members of our new decision rule class include (i) an integer for the decision variable index $j$; (ii) a Boolean recording whether $X_{j}$ is a continuous or categorical predictor; (iii) a double recording the value of the cutpoint $c$ for continuous $X_{j}$'s; and (iv) two sets storing the levels assigned to the left and right child of the node when $X_{j}$ is categorical.
To accommodate our new classes, we rewrote the function that determines the leaf node corresponding to a give $\bx.$
Briefly, given an instance of the rule class and $\bx,$ that function checks whether the decision variable is continuous or categorical.
If the variable is continuous, the function checks whether the corresponding entry in $\bx$ is less than the cutpoint.
Otherwise, for a categorical splitting variable, the function checks whether the relevant entry in $\bx$ is assigned to the left child of the node. 
We also introduced a separate function (\texttt{draw\_rule}) to draw new decision rules from the prior for use in the Metropolis-Hastings proposal.
After drawing the decision variable index $j$, the function checks whether $X_{j}$ is continuous or categorical and determines the set of available values $\calA.$
If $X_{j}$ is continuous, the function draws a cutpoint $c$ uniformly from the interval $\calA.$
If $X_{j}$ is categorical, the function draws a random subset of the discrete set $\calA$ and assigns it to the left child. 
See Appendix C for technical details about the implementation.

To summarize, whereas \textbf{BART} hard-coded information about the decision rule into its regression tree node class, we abstracted this information into a separate class.
Since we now store the levels assigned to the left and right child in the case of a categorical decision rule, this abstraction increases the memory footprint of our implementation.
However, we have observed that this overhead is often negligible in practice, even with many categorical levels.
Further, as we sketch in Section~\ref{sec:discussion}, such abstraction makes extending BART to use more complicated decision rules relatively straightforward.

While implementing our sampler, we noticed that \textbf{BART} performs many redundant calculations in each MCMC iteration.
Specifically, when \textbf{BART} grows a tree from or prunes a tree back to a particular node, it loops over all observations to determine which observations' decision-following paths reach that node.
Because at most two leaf nodes are changed during any tree update, the mapping from observations to leaf nodes does not change much iteration-to-iteration.
In other words, before updating a given regression tree, \textbf{BART} re-derives information that it had computed when updating the tree in the previous iterations.
In \textbf{flexBART}, we eliminated these redundancies by saving and manipulating a separate data structure that records which observations reach which leafs.
By maintaining these structure, we can eliminate unnecessary loops over the entire dataset, yielding substantial speed-ups at scale.
See Appendix C2 for more details. 

\subsection{Splitting a network-structured categorical predictor}
\label{sec:network_splits}

Figure~\ref{fig:philly_uniform_unordered} shows typical partitions of the Philadelphia census tracts induced by the BART prior when we randomly assign each categorical level to the left or right child instead of one-hot encoding. 
The corresponding regression trees promote partial pooling by forming several large clusters, each containing multiple tracts.
While these new partitions are a marked improvement over those in Figure~\ref{fig:philly_remove_one}, they are still not wholly satisfactory for our crime data. 
To wit, while Figure~\ref{fig:philly_crime_intro} suggests the presence of \textit{spatially contiguous} clusters of tracts with similar crime dynamics, all clusters in Figure~\ref{fig:philly_uniform_unordered} contain tracts that are geographically far apart.
That this is so is entirely expected: in assigning tracts independently to the children of a decision node, the BART prior described in Section~\ref{sec:cgm98_prior} does not leverage any spatial adjacency information!
To induce partitions with spatially contiguous clusters, we must change the decision rule prior.
Practically, using the backend of \textbf{flexBART}, the main work involves updating the function \texttt{draw\_rule}.

%Practically, within \textbf{flexBART}, it suffices to change the function that draws decision rules from the prior. 
To describe this modification, suppose we have a categorical predictor $X$ whose levels display a known similarity structure.
Suppose further that we would like our regression trees to partition the levels so that similar levels clustered together more often than not.
To achieve this, we form a network $\calG$ where each vertex corresponds to a distinct level of $X$ and an edge is drawn between vertices corresponding to similar levels.
Our goal, is to divide $\calG$ recursively into connected components.
%We assume that $\calG$ is connected and that our ultimate aim is to partition $\calG$ recursively into connected components.
In the context of our crime data, $\calG$'s vertices correspond to census tract and edges represent spatial adjacency.
%Clusters in Figure~\ref{fig:philly_spanning_tree} corresponds to connected subgraphs of $\calG.$

It suffices to describe a random process to partition a connected subgraph of $\calG$ into two connected components.
Specifically, suppose that in generating a regression tree from the prior that we have selected our network-structured categorical predictor $X$ as the decision variable.
Further, suppose that the set of available levels $\calA$ induces a connected subgraph $\calG[\calA]$ of $\calG.$ 
Unless $\calG[\calA]$ is a complete graph, independently assigning levels in $\calA$ to $\calC$ with a fixed probability tends not to partition $\calG[\calA]$ into two connected components.
We instead follow the three-step procedure illustrated in Figure~\ref{fig:mst_split}.
First, we draw a spanning tree of $\calG[\calA]$ using Wilson's algorithm \citep{Wilson1996}, which involves running a loop-erased random walk on the vertices of $\calG[\calA].$
Then, we delete a uniformly selected edge from the spanning tree, thereby partitioning the spanning tree into two connected components.
Finally, we set $\cutset$ to contain the vertices of one of these components. 
%Figure~\ref{fig:mst_split} illustrates our proposed process.

\begin{figure}[ht]
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_a}
\caption{}
\label{fig:mst_split_a}
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_b}
\caption{}
\label{fig:mst_split_b}
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_c}
\caption{}
\label{fig:mst_split_c}
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\centering
\includegraphics[width = \textwidth]{figures/mst_split_d}
\caption{}
\label{fig:mst_split_d}
\end{subfigure}
\caption{Cartoon illustration of our graph partitioning process. (a) Induced subgraph of levels available at a particular non-terminal node in the decision tree. (b) Uniformly drawn random spanning tree. (c) Deleting a uniformly selected edge (the edge $(2,8)$ in this case) from the spanning tree disconnects the tree and partitions the vertices into two subsets. (d) The subgraphs induced by the two vertex sets produced in (c) remain connected.}
\label{fig:mst_split}
\end{figure}

Embedding this process into the decision rule prior induces a prior over partitions of $\calG$ into connected components, which turns out to have full support.
That is, every partition of the network $\calG$ into connected components can be represented with a decision tree receiving positive prior probability.
%It turns out that this induced prior has full support, in the sense that every partition of the network into connect components receives positive prior probability.
In our motivating crime example, extending the BART prior in this way enables us to consider all spatially contiguous partitions of the census tracts. 


\begin{remark}
\label{remark:ust_process}
Forming spatially contiguous clusters by deleting spanning tree edges is an emerging idea in the spatial clustering literature \citep[see, e.g.,][]{Teixeira2015, Teixeira2019, LiSang2019, Luo2021}.
In the context of BART, \citet{Luo2021_BAST} and \citet{Luo2022} introduced a decision rule prior that is very similar to ours.
Whereas we were motivated by categorical predictors displaying network structure, their procedure recursively partitions a continuous manifold.
Briefly, they first triangulate the manifold and then form a graph capturing the adjacency relationships. 
%form a graph whose vertices corresponding to the triangular regions and whose edges encode adjacency relationships between the regions. 
Then they recursively remove edges from spanning trees of the graph to partition the manifold into contiguous regions.
\end{remark}





